GitBug-Actions: Building Reproducible Bug-Fix Benchmarks with GitHub Actions

Bug-fix benchmarks are fundamental in advancing various sub-fields of software engineering such as automatic program repair (APR) and fault localization (FL). A good benchmark must include recent examples that accurately reflect technologies and development practices of today. To be executable in the long term, a benchmark must feature test suites that do not degrade overtime due to, for example, dependencies that are no longer available. Existing benchmarks fail in meeting both criteria. For instance, Defects4J, one of the foremost Java benchmarks, last received an update in 2020. Moreover, full-reproducibility has been neglected by the majority of existing benchmarks. In this paper, we present GitBug-Actions: a novel tool for building bug-fix benchmarks with modern and fully-reproducible bug-fixes. GitBug-Actions relies on the most popular CI platform, GitHub Actions, to detect bug-fixes and smartly locally execute the CI pipeline in a controlled and reproducible environment. To the best of our knowledge, we are the first to rely on GitHub Actions to collect bug-fixes. To demonstrate our toolchain, we deploy GitBug-Actions to build a proof-of-concept Go bug-fix benchmark containing executable, fully-reproducible bug-fixes from different repositories. A video demonstrating GitBug-Actions is available at: https://youtu.be/aBWwa1sJYBs.

==> old-text.tex <==
old intro
Benchmarks of software bugs are valuable artifacts for the study of software engineering areas such as Automatic Program Repair (APR) and Fault Localization (FL). A benchmark of software bugs consists in a set of bugs collected from real-world projects or artifically generated sources. Each bug is associated with the buggy and fixed source code, supplementary metadata, and optionally an oracle, typically in the form of automated tests. Many benchmarks of software bugs were already proposed by the research community [], however many open challenges still remain. 

A core challenge for bugs benchmarks lies in scaling and ensuring regular updates. APR and FL benefit from having larger and richer datasets, especially when using Machine Learning. As the usage of Large Language Models (LLMs) has recently surged, it is crucial to have benchmarks that incorporate recent, non-training data. Additionally, the ever-evolving technological landscape in Software Engineering requires regular updates to benchmarks.
Defects4J~\cite{just2014defects4j} and Bears~\cite{madeiral2019bears} are examples of benchmarks that require manual validation of the bugs before they are added to the dataset, which results in scalability issues. The manual validation allows to filter only genuine bugs, and in the case of Defects4J, to minimize the source code diff to only contain relevant changes. BugSwarm~\cite{tomassi2019bugswarm} is a fully automated approach to collect a benchmark of bugs. However, the lack of a proper automated filter for bug candidates causes BugSwarm to fall into the pitfalls avoided by manual validation, with the majority of the dataset not being suitable for APR and FL~\cite{durieux2019critical}.

Another challenge is how to maintain the reproducibility of the oracles. Some datasets do not provide oracles \cite{csuvik2022fixjs}, which make them unusable for oracle-based methods (e.g. test-based patch generation) of APR and FL. Datasets containing oracles typically exhibit a decline over time in the number of reproducible bugs. Zhu and Rubio-González concluded from their experiments that automatically created benchmarks have reproducibility ranging from 26.6\% (Bugs.jar~\cite{saha2018bugs}) to 69.0\% (BugSwarm)~\cite{zhu2023reproducibility}. Only Defects4J, a manually-collected benchmark, had a higher reproducibility rate of 96.9\%~\cite{zhu2023reproducibility}. By adding dependency caching on a subset of BugSwarm's artifacts, Zhu and Rubio-González were able to increase the reproducibility from 69\% to a range between 81\% and 85\%. By selecting the artifacts from that subset able to be executed offline, the authors further increased the reproducibility to over 95\% \cite{zhu2023reproducibility}. One concern related to reproducibility is the storage required per bug sample. Since a Docker image is stored for each sample, Tomassi and Rubio-González report that BugSwarm uses 353 GB of disk space within a subset of 464 samples from the complete dataset~\cite{tomassi2019note}. With the average size increase rate of 5.1\% by adding dependency caching~\cite{zhu2023reproducibility}, we can estimate that BugSwarm uses around 819 MB\footnote{$\frac{353\textrm{GB} \times 1.051}{464} \times 1024\textrm{MB}$} per bug sample.

Finally, the last challenge we will consider is the generalization of the benchmarks. Hirsch and Hofer studied 73 benchmarks for evaluating debugging aproaches found in the literature~\cite{hirsch2022systematic}. We used the data found on their study~\cite{hirsch_thomas_2022_6670198} to conclude that out of the 73 benchmarks, only 13 (17.8\%) included scripts from more than one programming language. We also note that 58 out of the 73 (79.5\%) benchmarks include Java, Python, or C scripts, with the other 41 languages found in the dataset being present in only 23 benchmarks (31.5\%).

{\renewcommand{\arraystretch}{1.2} 
\begin{table}
\centering
\begin{tabular}{lllllll}
\hline
\textbf{Benchmark}      & \textbf{OS} & \textbf{BB} & \textbf{TS} & \textbf{HP} & \textbf{Scalable} & \textbf{FAIR} \\
\hline
10Y Bug-Fix DS & \checkmark & not sure &  &  & & 4.4 \\
\rowcolor{Gray}
BugSwarm       & \checkmark & $\sim$ &  &  &  & 4.3 \\
Code4Bench     &  & \checkmark &  &  &  & 4.4 \\
\rowcolor{Gray}
DataRaceBench  &  &  &  &  & & 4.5 \\
Defexts        & \checkmark &  &  &  &  & 3.3 \\
\rowcolor{Gray}
Denchmark      & \checkmark &  &  &  &  & 3.7 \\
Mandelbugs     & \checkmark &  &  &  &  & 2.4 \\
\rowcolor{Gray}
NFBugs         & \checkmark &  &  &  &  & 4.6 \\
NIST SAMATE    &  &  &  &  &  & 4.0 \\
\rowcolor{Gray}
QuixBugs       &  &  &  &  &  & 4.4 \\
SECbench       & \checkmark &  &  &  &  & 4.2 \\
\rowcolor{Gray}
SIR            & $\sim$ &  &  &  &  & 2.8 \\
TrainTicket    &  &  &  &  &  & 4.4 \\
\hline
\end{tabular}
\end{table}
}



